Dust reddening and extinction curves towards gamma-ray bursts at z > 4

Dust is known to be produced in the envelopes of AGB stars, the expanded shells of supernova (SN) remnants, and in situ grain growth in the ISM, although the corresponding efficiency of each of these dust formation mechanisms at different redshifts remains a topic of debate. During the first Gyr after the Big Bang, it is widely believed that there was not enough time to form AGB stars in high numbers, so that the dust at this epoch is expected to be purely from SNe, or subsequent grain growth in the ISM. The time period corresponding to z ~5-6 is thus expected to display the transition from SN-only dust to a mixture of both formation channels as we know it today. Here we aim to use afterglow observations of GRBs at redshifts larger than $z > 4$ in order to derive host galaxy dust column densities along their line-of-sight and to test if a SN-type dust extinction curve is required for some of the bursts. GRB afterglow observations were performed with the 7-channel GROND Detector at the 2.2m MPI telescope in La Silla, Chile and combined with data gathered with XRT. We increase the number of measured $A_V$ values for GRBs at z > 4 by a factor of ~2-3 and find that, in contrast to samples at mostly lower redshift, all of the GRB afterglows have a visual extinction of $A_V$ < 0.5 mag. Analysis of the GROND detection thresholds and results from a Monte-Carlo simulation show that, although we partly suffer from an observational bias against highly extinguished sight-lines, GRB host galaxies at 4 < z < 6 seem to contain on average less dust than at z ~ 2. Additionally, we find that all of the GRBs can be modeled with locally measured extinction curves and that the SN-like dust extinction curve provides a better fit for only two of the afterglow SEDs. For the first time we also report a photometric redshift of $z = 7.88$ for GRB 100905A, making it one of the most distant GRBs known to date.

==> authorlist.tex <==
\author{J.~Bolmer \inst{1,2,3} 
\and J. Greiner \inst{2}
\and T. Kr\"uhler \inst{2}
\and P. Schady \inst{2}
\and C. Ledoux \inst{1}
\and N. R. Tanvir \inst{4}
\and A. J. Levan \inst{5}
}

\institute{European Southern Observatory, Alonso de C\'{o}rdova 3107, Vitacura, Casilla 19001, Santiago 19, Chile\\
\email{[jbolmer,cledoux]@eso.org}
\and Max-Planck-Institut für extraterrestrische Physik, Giessenbachstraße, 85748 Garching, Germany\\
\email{[jcg,kruehler,pschady]@mpe.mpg.de}
\and Technische Universit\"{a}t M\"{u}nchen, Boltzmannstraße 2, D - 85748 Garching, Germany
\and University of Leicester, Department of Physics and Astronomy and  Leicester Institute of Space \& Earth Observation, University Road, Leicester, LE1 7RH, UK,
\email{nrt3@leicester.ac.uk}
\and Department of Physics, University of Warwick, Coventry, CV4 7AL, UK,
\email{a.j.levan@warwick.ac.uk}
}


%\offprints{J. Bolmer, \email{jbolmer@eso.org}}

==> definitions.tex <==
\newcommand{\farc}{\hbox{$\text{ }\!\!^{\prime\prime}$}} 
\newcommand{\ergA}{$\rm{erg\,cm^{-2}\,s^{-1}\,\AA^{-1}}$} 
\newcommand{\erg}{$\rm{erg\,cm^{-2}\,s^{-1}}$} 
\newcommand{\kms}{$\rm{km\,s^{-1}}\,$}

\newcommand{\griz}{$g' r' i' z'$}
\newcommand{\JHK}{$JHK_{\rm{s}}$}
\newcommand{\gK}{$g' r' i' z' JHK_{\rm{s}}$}
\newcommand{\msun}{$M_\odot$}

\newcommand\todo[1]{\textbf{(#1)}}

% Elements
\newcommand{\lya}{Ly$\alpha$} 
\newcommand{\lyb}{Ly$\beta$} 
\newcommand{\lyg}{Ly$\gamma$} 
\newcommand{\hb}{H$\beta$} 
\newcommand{\ha}{H$\alpha$} 
\newcommand{\hg}{H$\gamma$} 
\newcommand{\hi}{\ion{H}{i}} 
\newcommand{\hei}{[\ion{He}{i}]} 
\newcommand{\oi}{[\ion{O}{i}]} 
\newcommand{\sii}{[\ion{S}{ii}]} 
\newcommand{\siii}{[\ion{S}{iii}]}
\newcommand{\oii}{[\ion{O}{ii}]} 
\newcommand{\oiii}{[\ion{O}{iii}]}
\newcommand{\nii}{[\ion{N}{ii}]} 
\newcommand{\nv}{[\ion{N}{v}]} 
\newcommand{\neiii}{[\ion{Ne}{iii}]} 
\newcommand{\NIii}{[\ion{Ni}{ii}]} 
\newcommand{\feii}{\ion{Fe}{ii}}
\newcommand{\civ}{\ion{C}{iv}} 
\newcommand{\cii}{\ion{C}{ii}}
\newcommand{\mgi}{\ion{Mg}{i}} 
\newcommand{\mgii}{\ion{Mg}{ii}} 
\newcommand{\mgiv}{\ion{Mg}{iv}} 
\newcommand{\ali}{\ion{Al}{i}} 
\newcommand{\alii}{\ion{Al}{ii}} 
\newcommand{\aliii}{\ion{Al}{iii}} 
\newcommand{\SIi}{\ion{Si}{i}} 
\newcommand{\SIii}{\ion{Si}{ii}} 
\newcommand{\SIiii}{\ion{Si}{iii}} 
\newcommand{\SIiv}{\ion{Si}{iv}} 
\newcommand{\znii}{\ion{Zn}{ii}} 
\newcommand{\crii}{\ion{Cr}{ii}} 
\newcommand{\mnii}{\ion{Mn}{ii}} 
\newcommand{\tiii}{\ion{Ti}{ii}} 
\newcommand{\caii}{\ion{Ca}{ii}} 


==> table/fitres.tex <==
\begingroup
\renewcommand*{\arraystretch}{1.35}
\renewcommand{\tabcolsep}{0.52cm}

\begin{longtable}{c l c c l c l c c}
\caption{\label{tab:fitres}Results of fitting the NIR/optical to X-ray broadband SEDs}\\
\hline\hline
GRB		& $\beta_O$ & $\beta_X$ & $\text{E}_{\text{break}}$	& $\text{A}_V$(host)
		& $\text{N}_{\element[ ][]{H},\text{X}}$(host)	& model & $\chi^2_{\text{red}}$	\\
		\multicolumn{1}{c}{}	&\multicolumn{2}{c}{}	& (keV) &  (mag) & $(10^{21}\text{cm}^{-2})$ \\
\hline
\endfirsthead
\caption{continued.}\\
\hline\hline
GRB		& $\beta_O$ & $\beta_X$ & $\text{E}_{\text{break}}$	& $\text{A}_V$(host)
		& $\text{N}_{\element[ ][]{H},\text{X}}$(host)	& model & $\chi^2_{\text{red}}$	\\
		\multicolumn{1}{c}{}	&\multicolumn{2}{c}{}	& (keV) &  (mag) & $(10^{21}\text{cm}^{-2})$ \\
\hline
\endhead
\hline
\endfoot
  			& $-$	& $1.09^{+0.05}_{-0.06}$ & $-$ 		& $0.42^{+0.12}_{-0.11}$& $37^{+16}_{-13}$   & SMC 	& 1.17  \\
071025 PL	& $-$	& $1.14^{+0.07}_{-0.07}$ & $-$ 		& $0.65^{+0.17}_{-0.17}$& $42^{+17}_{-14}$   & LMC	& 1.17  \\
			& $-$	& $1.21^{+0.10}_{-0.11}$ & $-$ 		& $1.05^{+0.33}_{-0.34}$& $49^{+20}_{-17}$   & MW	& 1.37  \\
            & $-$	& $1.16^{+0.08}_{-0.08}$ & $-$ 		& $0.56^{+0.19}_{-0.17}$& $44^{+18}_{-15}$   & SN	& 1.13  \\
\hdashline
			& 0.77 	& $1.27^{+0.17}_{-0.08}$ & $0.01$	& $0.45^{+0.13}_{-0.14}$& $56^{+26}_{-17}$   & SMC 	& 1.11	\\
071025 BRPL & 0.80 	& $1.30^{+0.15}_{-0.06}$ & $0.01$	& $0.70^{+0.17}_{-0.22}$& $59^{+20}_{-15}$   & LMC	& 1.17	\\
			& 0.84	& $1.34^{+0.17}_{-0.12}$ & $0.01$	& $1.03^{+0.35}_{-0.59}$& $63^{+28}_{-19}$   & MW	& 1.50  \\
 			& 0.80	& $1.30^{+0.16}_{-0.07}$ & $0.01$	& $0.57^{+0.18}_{-0.21}$& $59^{+26}_{-15}$   & SN	& 1.16  \\
\hline
  			& $-$	& $1.08^{+0.05}_{-0.04}$ & $-$ 		& $<0.03$				& $250^{+300}_{-226}$& SMC 	& 1.25  \\
080129 PL	& $-$	& $1.08^{+0.05}_{-0.04}$ & $-$ 		& $<0.05$ 				& $250^{+300}_{-226}$& LMC	& 1.25  \\
			& $-$	& $1.08^{+0.05}_{-0.04}$ & $-$ 		& $<0.10$				& $250^{+310}_{-226}$& MW	& 1.25  \\
			& $-$	& $1.08^{+0.05}_{-0.04}$ & $-$ 		& $<0.05$				& $253^{+310}_{-225}$& SN	& 1.25  \\
\hdashline
			& 0.82 	& $1.32^{+0.32}_{-0.08}$ & $0.03$	& $0.07^{+0.06}_{-0.07}$& $337^{+418}_{-280}$& SMC 	& 1.67	\\
080129 BRPL & 0.77 	& $1.27^{+0.34}_{-0.04}$ & $0.01$	& $0.14^{+0.06}_{-0.14}$& $313^{+372}_{-204}$& LMC	& 1.42	\\
			& 0.89	& $1.39^{+0.22}_{-0.19}$ & $0.07$	& $0.16^{+0.18}_{-0.16}$& $370^{+359}_{-298}$& MW	& 1.41  \\
			& 0.77	& $1.27^{+0.34}_{-0.03}$ & $0.01$	& $0.13^{+0.05}_{-0.13}$& $315^{+355}_{-209}$& SN	& 1.09  \\
\hline          
  			& $-$	& $-$ 					 & $-$ 		& $-$					& $-$				& SMC	& >2.0  \\
080825B PL	& $-$	& $-$ 					 & $-$ 		& $-$					& $-$				& LMC	& >2.0  \\
			& $-$	& $-$ 					 & $-$ 		& $-$					& $-$				& MW	& >2.0  \\
			& $-$	& $-$ 					 & $-$ 		& $-$					& $-$				& SN	& >2.0  \\
\hdashline
			& 0.69 	& $1.19^{+0.19}_{-0.03}$ & $0.01$	& $0.05^{+0.02}_{-0.02}$& $12^{+69}_{-12}$  & SMC 	& 0.57  \\
080825B BRPL& 0.69 	& $1.19^{+0.19}_{-0.02}$ & $0.01$ 	& $0.07^{+0.03}_{-0.04}$& $15^{+75}_{-15}$  & LMC	& 0.59  \\
			& 0.79	& $1.29^{+0.12}_{-0.10}$ & $0.05$ 	& $0.04^{+0.12}_{-0.04}$& $21^{+88}_{-21}$  & MW	& 0.94  \\
            & 0.70	& $1.20^{+0.18}_{-0.04}$ & $0.01$	& $0.06^{+0.03}_{-0.06}$& $11^{+79}_{-11}$  & SN	& 0.60  \\
\hline
  			& $-$	& $0.59^{+0.02}_{-0.02}$ & $-$ 		& $<0.01$				& $10^{+47}_{-10}$  & SMC	& 0.82  \\
080913 PL	& $-$	& $0.59^{+0.02}_{-0.02}$ & $-$ 		& $<0.01$				& $10^{+47}_{-10}$  & LMC	& 0.82  \\
			& $-$	& $0.59^{+0.02}_{-0.02}$ & $-$ 		& $<0.01$				& $10^{+47}_{-10}$  & MW	& 0.82  \\
			& $-$	& $0.59^{+0.02}_{-0.02}$ & $-$ 		& $<0.01$ 				& $10^{+47}_{-10}$  & SN	& 0.82  \\
\hdashline
			& 0.24 	& $0.74^{+0.09}_{-0.02}$ & $0.01$	& $<0.07$				& $45^{+61}_{-41}$  & SMC 	& 1.20	\\
080913 BRPL & 0.24 	& $0.74^{+0.09}_{-0.02}$ & $0.01$	& $<0.15$				& $45^{+61}_{-41}$  & LMC	& 1.20	\\
			& 0.24	& $0.74^{+0.11}_{-0.02}$ & $0.01$	& $<0.18$				& $44^{+64}_{-39}$  & MW	& 1.20  \\
			& 0.24	& $0.74^{+0.13}_{-0.02}$ & $0.01$	& $<0.01$				& $45^{+61}_{-41}$  & SN	& 1.20  \\
\hline
  			& $-$	& $-$ 					 & $-$ 		& $-$					& $-$				& SMC	& >2.0  \\
080916CB PL	& $-$	& $-$ 					 & $-$ 		& $-$					& $-$				& LMC	& >2.0  \\
			& $-$	& $-$ 					 & $-$ 		& $-$					& $-$				& MW	& >2.0  \\
			& $-$	& $-$ 					 & $-$ 		& $-$					& $-$				& SN	& >2.0  \\
\hdashline
			& 0.40	& $0.90^{+0.12}_{-0.02}$ & $0.01$ 	& $0.01^{+0.03}_{-0.01}$& $50^{+46}_{-27}$  & SMC	& 0.95  \\ 
080916C BRPL& 0.40 	& $0.90^{+0.12}_{-0.02}$ & $0.01$ 	& $0.01^{+0.04}_{-0.01}$& $50^{+46}_{-26}$  & LMC 	& 0.95	\\
			& 0.40 	& $0.90^{+0.09}_{-0.02}$ & $0.01$ 	& $0.01^{+0.08}_{-0.01}$& $50^{+48}_{-24}$  & MW	& 0.97	\\
			& 0.41 	& $0.91^{+0.09}_{-0.02}$ & $0.01$ 	& $0.03^{+0.03}_{-0.03}$& $52^{+44}_{-28}$  & SN	& 0.91	\\
\hline
  			& $-$	& $0.89^{+0.02}_{-0.03}$ & $-$ 		& $0.08^{+0.03}_{-0.03}$& $1^{+25}_{-1}$ 	& SMC	& 1.48  \\
090205 PL	& $-$	& $0.90^{+0.03}_{-0.03}$ & $-$ 		& $0.13^{+0.04}_{-0.05}$& $3^{+26}_{-3}$  	& LMC	& 1.29  \\
			& $-$	& $0.93^{+0.03}_{-0.03}$ & $-$ 		& $0.25^{+0.08}_{-0.08}$& $4^{+26}_{-4}$  	& MW	& 1.33  \\
			& $-$	& $0.90^{+0.03}_{-0.03}$ & $-$ 		& $0.10^{+0.03}_{-0.03}$& $<27$     		& SN	& 1.37  \\
\hdashline
			& 0.86 	& $1.36^{+0.04}_{-0.26}$ & $1.24$ 	& $0.09^{+0.03}_{-0.03}$& $15^{+40}_{-15}$  & SMC 	& 1.23	\\
090205 BRPL & 0.88 	& $1.38^{+0.04}_{-0.24}$ & $1.24$ 	& $0.14^{+0.05}_{-0.05}$& $17^{+42}_{-17}$  & LMC	& 1.02	\\
			& 0.91	& $1.41^{+0.04}_{-0.04}$ & $1.30$	& $0.26^{+0.08}_{-0.09}$& $16^{+39}_{-16}$  & MW	& 1.14  \\
			& $-$	& $-$ 					 & $-$ 		& $-$					& $-$				& SN	& >2.0  \\
\hline
  			& $-$	& $0.88^{+0.04}_{-0.04}$ & $-$ 		& $0.09^{+0.09}_{-0.09}$& $101^{+50}_{-40}$ & SMC	& 0.90  \\
090423 PL	& $-$	& $0.90^{+0.06}_{-0.06}$ & $-$ 		& $0.16^{+0.17}_{-0.16}$& $107^{+53}_{-43}$ & LMC	& 0.90  \\
			& $-$	& $0.96^{+0.13}_{-0.12}$ & $-$ 		& $0.37^{+0.41}_{-0.37}$& $127^{+71}_{-57}$ & MW	& 0.90  \\
			& $-$	& $0.89^{+0.05}_{-0.05}$ & $-$ 		& $0.10^{+0.11}_{-0.10}$& $103^{+50}_{-41}$ & SN	& 0.90  \\
\hdashline
			& 0.56 	& $1.06^{+0.14}_{-0.02}$ & $0.01$ 	& $0.13^{+0.09}_{-0.09}$& $166^{+74}_{-48}$ & SMC 	& 0.93	\\
090423 BRPL & 0.58 	& $1.08^{+0.13}_{-0.04}$ & $0.01$ 	& $0.22^{+0.16}_{-0.16}$& $175^{+74}_{-51}$ & LMC	& 0.95	\\
			& 0.60	& $1.10^{+0.18}_{-0.02}$ & $0.01$ 	& $0.32^{+0.50}_{-0.32}$& $180^{+96}_{-63}$ & MW	& 1.07  \\
			& 0.57	& $1.07^{+0.14}_{-0.03}$ & $0.01$ 	& $0.14^{+0.10}_{-0.11}$& $168^{+58}_{-49}$ & SN	& 0.95  \\
\hline
  			& $-$	& $0.74^{+0.04}_{-0.03}$ & $-$ 		& $0.13^{+0.09}_{-0.08}$& $173^{+133}_{-101}$& SMC	& 1.19  \\
090429B PL	& $-$	& $0.81^{+0.08}_{-0.08}$ & $-$ 		& $0.37^{+0.23}_{-0.22}$& $212^{+144}_{-111}$& LMC	& 1.03  \\
			& $-$	& $-$ 					 & $-$ 		& $-$					& $-$				 & MW	& >2.0  \\
			& $-$	& $0.76^{+0.05}_{-0.05}$ & $-$ 		& $0.19^{+0.12}_{-0.12}$& $183^{+135}_{-104}$& SN	& 1.14  \\
\hdashline
			& 0.70 	& $1.20^{+0.05}_{-0.28}$ & $1.18$	& $0.14^{+0.12}_{-0.08}$& $294^{+245}_{-150}$& SMC 	& 0.56	\\
090429B BRPL& 0.77 	& $1.27^{+0.07}_{-0.29}$ & $1.22$	& $0.36^{+0.22}_{-0.22}$& $327^{+271}_{-160}$& LMC	& 0.55	\\
			& $-$	& $-$ 					 & $-$ 		& $-$					& $-$				 & MW	& >2.0  \\
			& 0.72	& $1.22^{+0.06}_{-0.27}$ & $1.19$ 	& $0.19^{+0.22}_{-0.14}$& $303^{+252}_{-152}$& SN	& 0.56  \\
\hline
 			& $-$	& $0.97^{+0.02}_{-0.02}$ & $-$ 		& $0.19^{+0.03}_{-0.03}$& $11^{+9}_{-7}$	& SMC	& 0.74 	\\
090516A	PL	& $-$	& $0.99^{+0.02}_{-0.02}$ & $-$ 		& $0.29^{+0.05}_{-0.05}$& $12^{+9}_{-7}$	& LMC	& 0.87  \\
			& $-$	& $1.01^{+0.03}_{-0.03}$ & $-$ 		& $0.44^{+0.09}_{-0.08}$& $13^{+9}_{-7}$	& MW	& 1.85  \\
 			& $-$	& $0.98^{+0.02}_{-0.02}$ & $-$ 		& $0.24^{+0.04}_{-0.05}$& $12^{+9}_{-7}$	& SN	& 1.15  \\
\hdashline
			& 0.65 	& $1.15^{+0.13}_{-0.01}$ & $0.01$	& $0.29^{+0.02}_{-0.02}$& $20^{+10}_{-6}$	& SMC 	& 0.81	\\
090516A BRPL& 0.99 	& $1.49^{+0.02}_{-0.02}$ & $>10$	& $0.29^{+0.05}_{-0.05}$& $12^{+9}_{-7}$	& LMC	& 0.91	\\
			& 1.01	& $1.51^{+0.03}_{-0.03}$ & $>10$ 	& $0.44^{+0.09}_{-0.08}$& $13^{+9}_{-7}$	& MW	& 1.93  \\
			& 0.98 	& $1.48^{+0.02}_{-0.02}$ & $>10$ 	& $0.24^{+0.04}_{-0.05}$& $12^{+9}_{-7}$	& SN	& 1.20  \\
\hline
 			& $-$	& $0.74^{+0.03}_{-0.03}$ & $-$ 		& $0.15^{+0.04}_{-0.05}$& $36^{+43}_{-27}$	& SMC 	& 0.47 	\\
100219A	PL	& $-$	& $0.76^{+0.04}_{-0.04}$ & $-$ 		& $0.23^{+0.07}_{-0.07}$& $38^{+44}_{-27}$	& LMC	& 0.53  \\
			& $-$	& $0.79^{+0.05}_{-0.05}$ & $-$ 		& $0.39^{+0.13}_{-0.14}$& $40^{+45}_{-28}$	& MW	& 1.24  \\
			& $-$	& $0.75^{+0.04}_{-0.04}$ & $-$ 		& $0.16^{+0.05}_{-0.05}$& $36^{+43}_{-27}$	& SN	& 0.65  \\
\hdashline
			& 0.74 	& $1.24^{+0.17}_{-0.35}$ & $>10$ 	& $0.15^{+0.11}_{-0.02}$& $36^{+76}_{-3}$	& SMC 	& 0.53	\\
100219A BRPL& 0.76 	& $1.26^{+0.17}_{-0.34}$ & $>10$ 	& $0.23^{+0.17}_{-0.03}$& $38^{+77}_{-4}$	& LMC	& 0.59	\\
			& 0.79	& $1.29^{+0.05}_{-0.05}$ & $>10$ 	& $0.39^{+0.13}_{-0.14}$& $40^{+45}_{-28}$	& MW	& 1.40  \\ 
 			& 0.75	& $1.25^{+0.04}_{-0.04}$ & $>10$ 	& $0.16^{+0.12}_{-0.03}$& $36^{+92}_{-11}$	& SN	& 0.74  \\
			& $-$	& $0.84^{+0.09}_{-0.04}$ & $-$ 		& $<0.19$ 				& $147^{+155}_{-108}$& SMC	& 0.44  \\
100905A	PL	& $-$	& $0.84^{+0.13}_{-0.04}$ & $-$ 		& $<0.34$				& $147^{+157}_{-108}$& LMC	& 0.43  \\
			& $-$	& $0.84^{+0.38}_{-0.04}$ & $-$ 		& $<1.26$				& $147^{+211}_{-108}$& MW	& 0.43  \\
			& $-$	& $0.84^{+0.04}_{-0.04}$ & $-$ 		& $<0.01$				& $147^{+155}_{-108}$& SN	& 0.43  \\
\hdashline
			& 0.61 	& $1.11^{+0.31}_{-0.15}$ & $0.05$ 	& $<0.25$ 				& $247^{+241}_{-159}$& SMC 	& 0.39	\\
100905A BRPL& 0.55 	& $1.05^{+0.40}_{-0.10}$ & $0.02$ 	& $<0.43$ 				& $226^{+263}_{-138}$& LMC	& 0.40	\\
			& 0.79	& $1.29^{+0.35}_{-0.33}$ & $0.93$ 	& $<1.50$ 				& $257^{+275}_{-169}$& MW	& 0.30  \\
			& 0.53	& $1.03^{+0.57}_{-0.08}$ & $0.02$ 	& $<0.28$ 				& $218^{+270}_{-70}$ & SN	& 0.40  \\
\hline
			& $-$	& $0.67^{+0.02}_{-0.03}$ & $-$ 		& $0.04^{+0.06}_{-0.04}$ & $11^{+14}_{-11}$ & SMC	& 1.73  \\
111008A	PL	& $-$	& $0.67^{+0.03}_{-0.03}$ & $-$ 		& $0.05^{+0.06}_{-0.05}$ & $11^{+14}_{-11}$ & LMC	& 1.78  \\
			& $-$	& $0.65^{+0.03}_{-0.01}$ & $-$ 		& $0.01^{+0.01}_{-0.01}$ & $9^{+13}_{-9}$ 	& MW	& 1.87  \\
			& $-$	& $0.68^{+0.03}_{-0.03}$ & $-$ 		& $0.06^{+0.05}_{-0.06}$ & $12^{+14}_{-11}$ & SN	& 1.73  \\
\hdashline
			& 0.35 	& $0.85^{+0.20}_{-0.01}$ & $0.01$	& $0.13^{+0.03}_{-0.08}$ & $28^{+27}_{-11}$ & SMC	& 1.42	\\
111008A BRPL& 0.36 	& $0.86^{+0.24}_{-0.01}$ & $0.01$	& $0.19^{+0.05}_{-0.16}$ & $29^{+35}_{-12}$ & LMC	& 1.62	\\
			& 0.63 	& $1.13^{+0.16}_{-0.16}$ & $1.94$	& $0.01^{+0.12}_{-0.01}$ & $17^{+49}_{-13}$ & MW	& 1.42	\\
    		& 0.38 	& $0.88^{+0.21}_{-0.02}$ & $0.01$	& $0.18^{+0.05}_{-0.15}$ & $30^{+12}_{-28}$ & SN	& 1.48	\\
\hline
     		& $-$	& $0.93^{+0.02}_{-0.02}$ & $-$ 		& $<0.02$				 & $8^{+14}_{-8}$ 	& SMC	& 1.33	\\
120712A PL	& $-$	& $0.93^{+0.02}_{-0.02}$ & $-$ 		& $<0.02$				 & $8^{+14}_{-8}$ 	& LMC 	& 1.33	\\
			& $-$	& $0.93^{+0.02}_{-0.02}$ & $-$ 		& $<0.02$ 			  	 & $8^{+14}_{-8}$ 	& MW 	& 1.33	\\
			& $-$	& $0.93^{+0.02}_{-0.02}$ & $-$ 		& $<0.03$				 & $8^{+14}_{-8}$ 	& SN 	& 1.33	\\
\hdashline            
			& 0.61 	& $1.11^{+0.25}_{-0.02}$ & $0.01$	& $0.08^{+0.03}_{-0.08}$ & $16^{+19}_{-10}$ & SMC	& 1.06	\\
120712A BRPL& 0.65 	& $1.15^{+0.27}_{-0.05}$ & $0.02$	& $0.11^{+0.11}_{-0.11}$ & $18^{+23}_{-13}$ & LMC 	& 1.23	\\
            & 0.83 	& $1.33^{+0.11}_{-0.13}$ & $0.43$	& $<0.11$				 & $27^{+18}_{-14}$ & MW 	& 1.38	\\
            & 0.70 	& $1.20^{+0.24}_{-0.10}$ & $0.04$	& $0.07^{+0.06}_{-0.07}$ & $21^{+21}_{-15}$ & SN 	& 1.23	\\
\hline
     		& $-$	& $1.01^{+0.02}_{-0.02}$ & $-$ 		& $<0.03$				 & $21^{+27}_{-19}$ & SMC 	& 0.65 	\\
130606A PL	& $-$	& $1.01^{+0.02}_{-0.02}$ & $-$ 		& $<0.04$				 & $21^{+27}_{-20}$ & LMC 	& 0.65	\\
			& $-$	& $1.01^{+0.03}_{-0.02}$ & $-$ 		& $<0.07$				 & $21^{+27}_{-20}$ & MW 	& 0.65	\\
			& $-$	& $1.01^{+0.02}_{-0.02}$ & $-$ 		& $<0.03$ 			  	 & $22^{+27}_{-20}$ & SN 	& 0.64	\\       
\hdashline            
			& 0.70 	& $1.20^{+0.13}_{-0.02}$ & $0.01$	& $0.07^{+0.03}_{-0.04}$& $42^{+31}_{-20}$ & SMC 	& 0.88	\\
130606A BRPL& 0.71 	& $1.21^{+0.16}_{-0.02}$ & $0.01$	& $0.12^{+0.02}_{-0.07}$& $43^{+19}_{-17}$ & LMC 	& 0.93	\\
            & 1.01 	& $1.51^{+0.20}_{-0.29}$ & $>10$ 	& $0.01^{+0.25}_{-0.01}$& $21^{+66}_{-7}$  & MW 	& 0.71	\\
            & 0.71 	& $1.21^{+0.13}_{-0.13}$ & $0.01$ 	& $0.09^{+0.02}_{-0.03}$& $42^{+32}_{-19}$ & SN 	& 0.88	\\
\hline      
    		& $-$	& $-$ 					 & $-$ 		& $-$					& $-$				 & SMC	& >2.0  \\
131117A PL	& $-$	& $-$ 					 & $-$ 		& $-$					& $-$				 & LMC	& >2.0  \\
    		& $-$	& $-$ 					 & $-$ 		& $-$					& $-$				 & MW	& >2.0  \\
            & $-$	& $-$ 					 & $-$ 		& $-$					& $-$				 & SN	& >2.0  \\
\hdashline
			& 0.35 	& $0.85^{+0.14}_{-0.02}$ & $0.01$	& $0.03^{+0.03}_{-0.03}$ & $10^{+15}_{-8}$   & SMC 	& 1.30	\\
131117A BRPL& 0.35 	& $0.85^{+0.14}_{-0.02}$ & $0.01$	& $0.05^{+0.04}_{-0.05}$ & $10^{+15}_{-10}$  & LMC 	& 1.30	\\
            & 0.38 	& $0.88^{+0.15}_{-0.04}$ & $0.01$	& $0.06^{+0.10}_{-0.06}$ & $11^{+17}_{-10}$  & MW 	& 1.40	\\
            & 0.36 	& $0.86^{+0.12}_{-0.02}$ & $0.01$	& $0.05^{+0.04}_{-0.05}$ & $11^{+15}_{-11}$  & SN 	& 1.17	\\
\hline
    		& $-$	& $0.85^{+0.02}_{-0.02}$ & $-$ 		& $0.07^{+0.03}_{-0.04}$& $18^{+20}_{-14}$   & SMC	& 1.21  \\
140311A PL	& $-$	& $0.86^{+0.03}_{-0.03}$ & $-$ 		& $0.10^{+0.05}_{-0.06}$& $18^{+20}_{-14}$   & LMC 	& 1.28	\\
			& $-$	& $0.85^{+0.03}_{-0.04}$ & $-$ 		& $0.11^{+0.10}_{-0.11}$& $17^{+20}_{-14}$   & MW 	& 1.61	\\
			& $-$	& $0.87^{+0.03}_{-0.03}$ & $-$ 		& $0.10^{+0.05}_{-0.05}$& $19^{+21}_{-14}$   & SN 	& 1.23	\\
\hdashline
			& 0.54 	& $1.04^{+0.05}_{-0.02}$ & $0.01$	& $0.16^{+0.03}_{-0.04}$& $33^{+28}_{-16}$ 	 & SMC 	& 1.82	\\
140311A BRPL& $-$	& $-$ 					 & $-$ 		& $-$					& $-$				 & LMC	& >2.0  \\
			& $-$	& $-$ 					 & $-$ 		& $-$					& $-$				 & MW	& >2.0  \\
			& $-$	& $-$ 					 & $-$ 		& $-$					& $-$				 & SN	& >2.0  \\
\hline
    		& $-$	& $-$ 					 & $-$ 		& $-$					& $-$				 & SN	& >2.0  \\
140428A PL	& $-$	& $-$ 					 & $-$ 		& $-$					& $-$				 & LMC	& >2.0  \\
			& $-$	& $0.91^{+0.07}_{-0.08}$ & $-$ 		& $0.32^{+0.19}_{-0.20}$& $<18$ 	 		 & MW 	& 1.94	\\
 			& $-$	& $0.87^{+0.05}_{-0.05}$ & $-$ 		& $0.13^{+0.08}_{-0.08}$& $<16$ 	 		 & SN 	& 1.81	\\
\hdashline
			& 0.80 	& $1.30^{+0.09}_{-0.29}$ & $0.87$ 	& $0.10^{+0.12}_{-0.04}$& $6^{+35}_{-6}$ 	 & SMC 	& 1.56	\\
140428A BRPL& 0.82 	& $1.32^{+0.07}_{-0.31}$ & $0.86$ 	& $0.16^{+0.21}_{-0.12}$& $7^{+36}_{-7}$ 	 & LMC 	& 1.46	\\
			& 0.86 	& $1.36^{+0.09}_{-0.30}$ & $0.93$	& $0.30^{+0.33}_{-0.23}$& $7^{+38}_{-7}$     & MW 	& 1.43	\\
 			& 0.74 	& $1.24^{+0.15}_{-0.24}$ & $0.24$	& $0.15^{+0.13}_{-0.11}$& $16^{+30}_{-16}$   & SN 	& 1.16	\\
\hline
  			& $-$	& $0.77^{+0.04}_{-0.03}$ & $-$ 		& $<0.10$				& $<48$ 	 	 	 & SMC 	& 0.61	\\
140515A PL  & $-$	& $0.77^{+0.05}_{-0.03}$ & $-$ 		& $<0.15$ 				& $<48$ 	 	 	 & LMC 	& 0.61	\\	 
			& $-$	& $0.77^{+0.07}_{-0.03}$ & $-$ 		& $<0.22$ 				& $<48$   		 	 & MW 	& 0.61	\\
			& $-$	& $0.77^{+0.03}_{-0.03}$ & $-$ 		& $<0.10$				& $<48$   		 	 & SN 	& 0.61	\\
\hdashline
			& 0.77 	& $1.27^{+0.17}_{-0.37}$ & $0.01$ 	& $<0.07$				& $<80$   		 	 & SMC 	& 0.74	\\
140515A BRPL& 0.44 	& $0.94^{+0.13}_{-0.03}$ & $0.01$	& $<0.10$				& $<80$ 		 	 & LMC 	& 0.74	\\
			& 0.77 	& $1.27^{+0.18}_{-0.37}$ & $0.01$ 	& $<0.14$				& $<80$   		 	 & MW 	& 0.74	\\   
			& 0.77 	& $1.27^{+0.03}_{-0.03}$ & $0.01$	& $<0.10$				& $<80$ 		 	 & SN 	& 0.74	\\
\hline
 			& $-$	& $0.61^{+0.04}_{-0.04}$ & $-$ 		& $0.12^{+0.08}_{-0.08}$ & $<12$ 	 		& SMC 	& 0.84	\\
140614A PL 	& $-$	& $0.63^{+0.05}_{-0.05}$ & $-$		& $0.19^{+0.12}_{-0.11}$ & $<12$ 	 		& LMC 	& 0.83	\\
        	& $-$	& $0.64^{+0.06}_{-0.07}$ & $-$		& $0.28^{+0.20}_{-0.24}$ & $<12$ 	 		& MW 	& 0.95	\\
            & $-$	& $0.64^{+0.05}_{-0.05}$ & $-$		& $0.16^{+0.10}_{-0.10}$ & $<12$ 	 		& SN 	& 0.79	\\
\hdashline
        	& 0.60 	& $1.10^{+0.05}_{-0.05}$ & $1.89$	& $0.11^{+0.17}_{-0.05}$ & $<28$ 			& SMC 	& 0.65 	\\      
140614A BRPL& 0.60	& $1.10^{+0.06}_{-0.05}$ & $1.91$	& $0.16^{+0.27}_{-0.05}$ & $<20$	 		& LMC 	& 0.67 	\\
        	& 0.50 	& $1.00^{+0.27}_{-0.22}$ & $0.18$	& $0.32^{+0.31}_{-0.32}$ & $10^{+27}_{-10}$ & MW 	& 1.08	\\
            & 0.32 	& $0.82^{+0.35}_{-0.06}$ & $0.01$	& $0.27^{+0.09}_{-0.19}$ & $<20$ 			& SN 	& 0.70	\\       
\hline
 			& 0.83 	& $1.33^{+0.02}_{-0.02}$ & $-$ 		& $<0.01$				 & $64^{+30}_{-20}$ & SMC 	& 1.30	\\
151027B PL 	& 0.83 	& $1.33^{+0.02}_{-0.02}$ & $-$		& $<0.02$				 & $64^{+30}_{-20}$ & LMC 	& 1.30	\\
        	& 0.83 	& $1.33^{+0.02}_{-0.02}$ & $-$		& $<0.03$				 & $64^{+30}_{-20}$ & MW 	& 1.30	\\
          	& 0.83 	& $1.33^{+0.02}_{-0.02}$ & $-$		& $<0.01$				 & $64^{+30}_{-20}$ & SN 	& 1.30	\\
\hdashline
        	& 0.50 	& $1.00^{+0.08}_{-0.02}$ & $0.01$	& $0.06^{+0.03}_{-0.04}$ & $80^{+39}_{-23}$ & SMC	& 1.17	\\
151027B BRPL& 0.50 	& $1.00^{+0.08}_{-0.02}$ & $0.01$	& $0.10^{+0.05}_{-0.06}$ & $81^{+38}_{-23}$ & LMC 	& 1.16	\\
        	& 0.51 	& $1.01^{+0.12}_{-0.01}$ & $0.01$	& $0.15^{+0.05}_{-0.12}$ & $82^{+40}_{-20}$ & MW 	& 1.30	\\
        	& 0.51 	& $1.01^{+0.07}_{-0.02}$ & $0.01$	& $0.09^{+0.04}_{-0.05}$ & $85^{+39}_{-22}$ & SN 	& 1.05	\\
\hline
 			& $-$	& $0.73^{+0.04}_{-0.04}$ & $-$ 		& $0.36^{+0.06}_{-0.09}$ & $3^{+7}_{-3}$  	& SMC 	& 1.65	\\
151112A PL 	& $-$	& $0.77^{+0.04}_{-0.05}$ & $-$		& $0.56^{+0.11}_{-0.12}$ & $6^{+8}_{-6}$  	& LMC 	& 1.49	\\
        	& $-$	& $0.84^{+0.05}_{-0.06}$ & $-$		& $0.96^{+0.17}_{-0.18}$ & $10^{+8}_{-7}$ 	& MW 	& 1.40	\\
        	& $-$	& $0.78^{+0.03}_{-0.05}$ & $-$		& $0.48^{+0.06}_{-0.15}$ & $6^{+8}_{-6}$  	& SN 	& 1.54	\\
\hdashline
        	& 0.68 	& $1.18^{+0.17}_{-0.22}$ & $1.32$ 	& $0.33^{+0.12}_{-0.08}$ & $11^{+25}_{-3}$  & SMC  	& 0.89  \\
151112A BRPL& 0.72 	& $1.22^{+0.05}_{-0.06}$ & $1.36$ 	& $0.50^{+0.21}_{-0.11}$ & $12^{+26}_{-14}$ & LMC 	& 0.86	\\
        	& 0.78 	& $1.28^{+0.18}_{-0.28}$ & $1.45$ 	& $0.84^{+0.42}_{-0.19}$ & $15^{+27}_{-0}$  & MW 	& 0.96	\\
        	& 0.71 	& $1.13^{+0.06}_{-0.07}$ & $1.35$ 	& $0.41^{+0.11}_{-0.12}$ & $12^{+10}_{-8}$  & SN 	& 0.92	\\ \hline
\end{longtable}
\tablefoot{Columns 2-7 are the spectral slope in the NIR/optical ($\beta_O$) and the X-rays ($\beta_X$),
	the energy of the spectral break ($\text{E}_{\text{break}}$), the visual extinction ($\text{A}_V$)
    and neutral hydrogen column density ($\text{N}_{\element[ ][]{H},\text{X}}$) from the host galaxy,
    the used model and the goodness of the fit ($\chi^2_{\text{red}}$).}
\endgroup





